Streaming Graph Algorithms in the Massively Parallel Computation Model

We initiate the study of graph algorithms in the streaming setting on massive distributed and parallel systems inspired by practical data processing systems. The objective is to design algorithms that can efficiently process evolving graphs via large batches of edge insertions and deletions using as little memory as possible. We focus on the nowadays canonical model for the study of theoretical algorithms for massive networks, the Massively Parallel Computation (MPC) model. We design MPC algorithms that efficiently process evolving graphs: in a constant number of rounds they can handle large batches of edge updates for problems such as connectivity, minimum spanning forest, and approximate matching while adhering to the most restrictive memory regime, in which the local memory per machine is strongly sublinear in the number of vertices and the total memory is sublinear in the graph size. These results improve upon earlier works in this area which rely on using larger total space, proportional to the size of the processed graph. Our work demonstrates that parallel algorithms can process dynamically changing graphs with asymptotically optimal utilization of MPC resources: parallel time, local memory, and total memory, while processing large batches of edge updates.

==> algorithms.tex <==
\section{Pseudocodes from Section~\ref{sec:connect-single}}\label{app:pseudocodes}
\label{sec:algorithms}
\begin{algorithm}[H]
\caption{\textsc{Connectivity} $(e=\{u,v\})$}
\label{alg:conn}

\textbf{Initialization:} The spanning forest consists of $n$ components where each component corresponds to a vertex of the graph.  No sketch for the components is stored and those will be initiated over updates.

\textbf{Operation:} Based on the instruction whether insertion of an edge, deletion of an edge, or reporting of the current spanning tree call \textsc{Insert}, \textsc{Delete}, or \textsc{Query}; respectively.
\end{algorithm}

\begin{algorithm}[H]
\caption{\textsc{Insert} $(e=\{u,v\})$  }
\label{algo:insert}
   Update the sketches $S_{u}$ and $S_v$ with the information that $\{u,v\}$ is inserted.

\If{$C[u]=C[v]$}
{
No change to $F$.

}
\Else
{
    Add  $\{u,v\}$ to $F$. \ {\small \textit{// Note that components $C[u]$, $C[v]$ are merged to form a bigger component}}

    Update the component id of all vertices in $C_u$ or $C_v$ as follows:

    \lIf{$C[u] < C[v]$}{the components ids of all the vertices in $C_v$ are changed to $C[u]$}
    \lElse{the component ids of all the vertices in $C_u$ are changed to $C[v]$}

   % Initiate a sketch $S_{u}$ of $\mathbf{X}_{{u}}$ and insert the edge $\{u,v\}$.
}
\end{algorithm}
%\newpage
\begin{algorithm}[H]
\caption{\textsc{Delete} $(e=\{u,v\})$}
\label{alg:delete}

// \textit {\small In this case $C[u]=C[v]$}

  Update the sketches $S_{u}$ and $S_v$ with the information that $\{u,v\}$ is deleted.

\If {$\{u, v\}$ is not in $F$}
{
   No need to do anything.
}
\ElseIf{$\{u,v\}$ is in $F$}
{
   Determine the sketch ${S}_{Z_u}$ of ${X}_{Z_u}$ by merging the sketches of all the vertices in $Z_u$.

    Use the sketch ${S}_{Z_u}$ to find a possible replacement edge between $Z_u$ and $Z_v$.

    \If {$S_{Z_u}$ reports $\perp$}
    {
        {\small \textit{ // In this case, there is no edge between $Z_u$ to $Z_v$}.}

        Update the component ids of the vertices in $Z_u \cup Z_v$ as follows:

        \quad $\triangleright$ all vertices in $Z_u$ are assigned a component id $\min_{x \in Z_u} C[x]$ and all vertices in $Z_v$ are assigned a component id $\min_{x \in Z_v} C[x]$.
        \label{algo:delete-line-id}
    }
    \ElseIf{$S_{Z_u}$ reports an edge $\{a,b\}$}
    {
        %Let $a$ is in $Z_u$ and $b$ is in $Z_v$.
        Add $\{a,b\}$ to $F$.
    }
}
\end{algorithm}
\begin{algorithm}[H]
\caption{\textsc{Query}}  \label{alg:query}
 Report the spanning forest $F$ stored by the data structure.
\end{algorithm}

==> prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}

%\subsection{Notations}
\label{subsec:notation}
Let $[n]$ denote the set $\{1,\ldots, n\}$. Let $G = (V(G),E(G))$ denote an \emph{undirected} graph $G$ with vertex set $V(G)$ and edge set $E(G)$. When $G$ is clear from the context, we may denote $V(G)$ and $E(G)$ by $V$ and $E$, respectively. %We consider undirected graphs in this paper.
Throughout the paper, $n$ denotes the number of vertices in $G$. For an edge $e$, $G \cup \{e\}$ denotes the graph with vertex set $V(G)$ and edge set $E(G) \cup \{e\}$. $G \setminus \{e\}$ denotes the graph with vertex set $V(G)$ and edge set $E(G) \setminus \{e\}$. A subgraph $F$ of a graph $G$ is called a \emph{spanning forest} if it is a collection of disjoint trees that cover all the vertices of $G$ without forming cycles. An edge present in a spanning forest is referred to as a \emph{tree edge} and all other edges in the graph are called \emph{non-tree edges}. For a vector $\mathbf{X}$, $\mathbf{X}_j$ denotes the $j$-th coordinate of $\mathbf{X}$ and $\ell_0(\mathbf{X})$ is the standard $\ell_0$ norm of vector $\mathbf{X}$, i.e., the number of non-zero elements in vector $\mathbf{X}$. When we say an event holds \emph{with high probability} (w.h.p.), we mean that the event holds with probability at least $1-1/\poly(n)$.
%
\subsection{Preliminaries on sketching}
\label{subsec:sketching}

Graph sketching provides a powerful approach to summarize and approximate the structural properties of graphs without needing to store or process the entire graph. Graph sketching algorithms typically operate incrementally as the graph stream arrives, updating the sketch accordingly. By constructing compact graph sketches, it becomes possible to approximate key graph properties.

First, in the following lemma, we discuss the $\ell_0$ sketching result of a vector in streaming. Then we use it to discuss sketching the neighborhood of the vertices in a graph.
\begin{lemma}[\cite{CJ19}]
\label{lem:ell0}
There exists a dynamic streaming algorithm that receives updates to a vector $\mathbf{X}\in \{-1,0,1\}^{N}$, stores a sketch $S$ of $\Oh(\log ^3 N)$ bits for $\mathbf{X}$, and works as follows with probability $1-1/\poly (N)$: upon a query to sketch $S$ we either get $\perp$ or an index $i \in [N]$ randomly from the set $\{j \in [N]:\mathbf{X}_j\neq 0\}$ depending on whether $\ell_0(\mathbf{X})=0$ or not.
\end{lemma}
%
\begin{remark}
Note that the sketch in Lemma~\ref{lem:ell0} is \emph{linear} or \emph{mergable} i.e., let $S_1$ and $S_2$ be the linear sketches of vectors $\mathbf{X}_1$ and $\mathbf{X}_2$, then $S_1+S_2$ is also a sketch of $\mathbf{X_1}+\mathbf{X_2}$. This makes the updates in the streaming algorithm of Lemma~\ref{lem:ell0} easy.
\end{remark}
Using Lemma~\ref{lem:ell0}, we discuss the sketching results we will be using in this paper. To start, let $G$ be a graph with $V(G)=\{v_1,\ldots,v_n\}$.  For a vertex $v_i \in V(G)$, consider a vector $\mathbf{X}_{v_i}$ in $\{-1,0,1\}^{n \choose 2}$ whose each entry is of the form $\{j,k\} \in {[n] \choose 2}$ such that
\[ \mathbf{X}_{v_i} (\{v_j,v_k\})=\begin{cases}
      +1, &  \{v_j,v_k\}\in E(G)~\mbox{and}~i=\max\{j,k\}   \\
      -1, &  \{v_j,v_k\}\in E(G)~\mbox{and}~i=\min\{j,k\}   \\
      0, & \mbox{otherwise.}
   \end{cases}
\]
% \For a non-empty subset $S$ of $V$, let us define the neighborhood set of $S$ as $N_G(S) := \{i \in [n]: \mbox{$S \cap N_G(i) \neq \emptyset$ and $i \notin S$} \}.$ The indicator vector for $N_G(S)$ is the vector $\mathbf{x}_{S} \in \{0,1\}^n$ whose $i$-th bit $x_i$ is set as follows:

% \[ x_i =\begin{cases}
%       1 & i \in N_G(S) \\
%       0 & otherwise
%    \end{cases}
% \]

% Assume that  $N_G(S) \neq \emptyset$ or equivalently $E_S  \neq \emptyset$.
 %(over one pass to the edges of $G$) such that  the following holds :
For a subset $S \subseteq V(G)$, let us define $\mathbf{X}_S:=\sum\limits_{v \in S}\mathbf{X}_v$. Let $E(A, B)$ be the set of edges having one endpoint in $A$ and the other in $B$.

Now, consider the following lemma that gives a connection between the vector $\mathbf{X}_A$ and the set of edges in $E(A, V\setminus A)$, where $A$ is a subset of $V(G)$.
\begin{lemma}[\cite{AGM12}]
Let us consider $A \subseteq V(G)$. Then $\size{E(A,V \setminus A)}=\ell_o(\mathbf{X}_A)$. Also, for any $\{j,k\} \in {[n] \choose 2}$, $\mathbf{X}_{A}(\{j,k\})=\pm 1$ if and only if $ \{j,k\} \in E(A,V\setminus A)$.
\end{lemma}
Next, we consider some lemmas about sketching the neighborhood of a vertex (Lemma~\ref{lem:sketch1}) or a set of vertices (Lemma~\ref{lem:sketch}). All three lemmas follow from Lemma~\ref{lem:ell0}. However, we have stated them in different forms that will be useful in our proofs.
%
\begin{lemma}\label{lem:sketch1}
%Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
Let $v$ be a vertex of $G$. There exists a one-pass streaming algorithm that stores an $\Oh(\log^3 n)$ size sketch $S_{v}$ of $\mathbf{X}_v$ such that w.h.p. the algorithm does the following:
\begin{itemize}
\item when $E(\{v\}, V \setminus \{v\}) =\emptyset$,  i.e., $v$ is a singleton vertex, we get~$\perp$;
\item  $E(\{v\}, V \setminus \{v\}) \neq \emptyset$, we get  a random edge from $E(\{v\}, V \setminus \{v\})$, i.e., a random edge with $v$ as an endpoint.
\end{itemize}
Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
\end{lemma}

% \begin{proof}
% This follows from \Cref{lem:ell0} where our objective is to store a sketch of the vector $\mathbf{X}_v$. Note that any update to the neighborhood of $v$ can be thought of as an update to the vector $\mathbf{X}_v$.
% \end{proof}

\begin{lemma}\label{lem:sketch}
%Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
There exists a one-pass streaming algorithm that stores an $\Oh(\log^3 n)$ size  sketch $S_{v}$ of $\mathbf{X}_v$ for each $v \in V(G)$ such that w.h.p. the algorithm does the following for a given subset $A \subset V(G)$:
\begin{itemize}
    \item reports $\perp$ when $E(A, V \setminus A)=\emptyset$
    \item reports a random edge from $E(A, V\setminus A)$ when $E(A, V \setminus A) \neq \emptyset$.
\end{itemize}
Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
\end{lemma}

\color{black}

% \begin{proof}
% Let us consider the sketch $S_v$ for $\mathbf{X}_v$ as guaranteed by the algorithm \Cref{lem:sketch1}. Clearly, the space complexity of the algorithm is $\Oh(n \log ^3 n)$. For $A \subseteq V(G)$, let us consider the sketch $S_A= \sum_{v \in A}S_v$. Recall that $S_v$ is the sketch for $\mathbf{X_v}$, $\mathbf{X}_A=\sum_{v \in A}\mathbf{X}_v$, and sketches are linear. So, $S_A$ is a sketch for $\mathbf{X}_A$ such that the desired properties hold (as mentioned in the statement) w.h.p.
% % The correctness for a single update follows from the $\ell_0$ sampling result\anish{which result?} by maintaining a sketch of the vector $\mathbf{X}_{{AB}}$. Hence, the lemma follows by applying the union bound over all the updates.
% \end{proof}

%\gopi{We think that the above lemma is correct.}
%When we insert an edge $e$ in $E(A, B)$, then $X_{{AB}}$ is changed. So, for simplicity, we say that we insert (delete) an edge $e$ to (from) the sketch of $\mathbf{X}_{{AB}}$ to mean that the sketch of $X_{{AB}}$ is updated to take care of the event that $e$ is inserted (deleted).

% \begin{lemma}\label{lem:sketch-A-B}
% %Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
% Let $A$ and $B$ be disjoint subsets of $V(G)$.
% There exists a one-pass streaming algorithm that  stores an $\Oh(\log^3 n)$ size  sketch for $E(A,B)$ such that w.h.p. the algorithm does the following:
% \begin{itemize}
%     \item reports $\perp$ when $E(A, B)=\emptyset$
%     \item reports a random edge from $E(A, B)$ when $E(A, B) \neq \emptyset$.
% \end{itemize}
% Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
% \end{lemma}
% \begin{proof}
%     Follows from \Cref{lem:ell0}.
% \end{proof}

%We denote by $[n]$ the set $\{1,\ldots, n\}$. Let $G=(V(G),E(G))$ denote a graph $G$ with vertex set $V(G)$ and edge set $E(G)$. When the graph $G$ is clear from the context, we sometimes denote $V(G)$ and $E(G)$ by $V$ and $E$, respectively. We consider undirected graphs in this paper. Throughout the paper, $n$ denotes the number of vertices in $G$. For an edge $e$, $G \cup \{e\}$ denotes the graph with vertex set $V(G)$ and edge set $E(G) \cup \{e\}$. $G \setminus \{e\}$ denotes the graph with vertex set $V(G)$ and edge set $E(G) \setminus \{e\}$. A subgraph $F$ of a graph $G$ is called a spanning forest if it is a collection of disjoint trees that cover all the vertices of $G$ without forming cycles. An edge present in a spanning forest is referred to as a tree edge and all other edges in the graph are called non-tree edges. For a vector $\mathbf{X}$, $\mathbf{X}_j$ denotes the $j$-th coordinate of $\mathbf{X}$ and $\ell_0(\mathbf{X})$ is the standard $\ell_0$ norm of vector $\mathbf{X}$, i.e., the number of non-zero elements in vector $\mathbf{X}$. When we say an event holds with high probability (w.h.p. in short), we mean that the event holds with probability at least $1-1/\poly(n)$.

% \subsection{Sketching}
% \label{subsec:sketching}
% Graph sketching provides a powerful approach to summarize and approximate the structural properties of graphs without needing to store or process the entire graph. Graph sketching algorithms typically operate incrementally as the graph stream arrives, updating the sketch accordingly. By constructing compact graph sketches, it becomes possible to approximate key graph properties.

% First, in the following lemma, we discuss the $\ell_0$ sketching result of a vector in streaming. Then we use it to discuss sketching the neighborhood of the vertices in a graph.
% \begin{lemma}[\cite{CJ19}]
% \label{lem:ell0}
% There exists a dynamic streaming algorithm that receives updates to a vector $\mathbf{X}\in \{-1,0,1\}^{N}$, stores a sketch $S$ of $\Oh(\log ^3 N)$ bits for $\mathbf{X}$, and works as follows with probability $1-1/\poly (N)$: upon a query to sketch $S$ we either get $\perp$ or an index $i \in [N]$ randomly from the set $\{j \in [N]:\mathbf{X}_j\neq 0\}$ depending on whether $\ell_0(\mathbf{X})=0$ or not.
% \end{lemma}
% %
% \begin{remark}
% Note that the sketch in \Cref{lem:ell0} is \emph{linear} or \emph{mergable} i.e., let $S_1$ and $S_2$ be the linear sketches of vectors $\mathbf{X}_1$ and $\mathbf{X}_2$, then $S_1+S_2$ is also a sketch of $\mathbf{X_1}+\mathbf{X_2}$. This makes the updates in the streaming algorithm of \Cref{lem:ell0} easy.
% \end{remark}
% Using \Cref{lem:ell0}, we discuss the sketching results we will be using in this paper. To begin with, let $G$ be a graph with $V(G)=\{v_1,\ldots,v_n\}$.  For a vertex $v_i \in V(G)$, consider a vector $\mathbf{X}_{v_i}$ in $\{-1,0,1\}^{n \choose 2}$ whose each entry is of the form $\{j,k\} \in {[n] \choose 2}$ such that
% \[ \mathbf{X}_{v_i} (\{v_j,v_k\})=\begin{cases}
%       +1, &  \{v_j,v_k\}\in E(G)~\mbox{and}~i=\max\{j,k\}   \\
%       -1, &  \{v_j,v_k\}\in E(G)~\mbox{and}~i=\min\{j,k\}   \\
%       0, & \mbox{otherwise.}
%    \end{cases}
% \]
% % \For a non-empty subset $S$ of $V$, let us define the neighborhood set of $S$ as $N_G(S) := \{i \in [n]: \mbox{$S \cap N_G(i) \neq \emptyset$ and $i \notin S$} \}.$ The indicator vector for $N_G(S)$ is the vector $\mathbf{x}_{S} \in \{0,1\}^n$ whose $i$-th bit $x_i$ is set as follows:

% % \[ x_i =\begin{cases}
% %       1 & i \in N_G(S) \\
% %       0 & otherwise
% %    \end{cases}
% % \]

% % Assume that  $N_G(S) \neq \emptyset$ or equivalently $E_S  \neq \emptyset$.
%  %(over one pass to the edges of $G$) such that  the following holds :
% For a subset $S \subseteq V(G)$, let us define $\mathbf{X}_S:=\sum\limits_{v \in S}\mathbf{X}_v$. Let $E(A, B)$ be the set of edges having one endpoint in $A$ and the other endpoint in $B$.

% Now, consider the following lemma that gives a connection between the vector $\mathbf{X}_A$ and the set of edges in $E(A, V\setminus A)$, where $A$ is a subset of $V(G)$.
% \begin{lemma}[\cite{AGM12}]
% Let us consider $A \subseteq V(G)$. Then $\size{E(A,V \setminus A)}=\ell_o(\mathbf{X}_A)$. Also, for any $\{j,k\} \in {[n] \choose 2}$, $\mathbf{X}_{A}(\{j,k\})=\pm 1$ if and only if $ \{j,k\} \in E(A,V\setminus A)$.
% \end{lemma}
% Next, we consider three different lemmas that talk about sketching the neighborhood of a vertex (\Cref{lem:sketch1}), or a set of vertices (\Cref{lem:sketch}), or between two sets of vertices (\Cref{lem:sketch-A-B}). All three lemmas follow from \Cref{lem:ell0}. However, we have stated them in different forms that will be useful in our proofs.
% %
% \begin{lemma}
% \label{lem:sketch1}
% %Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
% Let $v$ be a vertex of $G$. There exists a one-pass streaming algorithm that  stores an $\Oh(\log^3 n)$ size sketch $S_{v}$ of $\mathbf{X}_v$ such that w.h.p. the algorithm does the following:
% \begin{itemize}
% \item when $E(\{v\}, V \setminus \{v\}) =\emptyset$,  i.e., $v$ is a singleton vertex, we get  $\perp$;
% \item  $E(\{v\}, V \setminus \{v\}) \neq \emptyset$, we get  a random edge from $E(\{v\}, V \setminus \{v\})$, i.e., a random edge with $v$ as an endpoint.
% \end{itemize}
% Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
% \end{lemma}

% \begin{proof}
% This follows from \Cref{lem:ell0} where our objective is to store a sketch of the vector $\mathbf{X}_v$. Note that any update to the neighborhood of $v$ can be thought of as an update to the vector $\mathbf{X}_v$.
% \end{proof}

% \begin{lemma}\label{lem:sketch}
% %Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
% There exists a one-pass streaming algorithm that stores an $\Oh(\log^3 n)$ size  sketch $S_{v}$ of $\mathbf{X}_v$ for each $v \in V(G)$ such that w.h.p. the algorithm does the following for a given subset $A \subset V(G)$:
% \begin{itemize}
%     \item reports $\perp$ when $E(A, V \setminus A)=\emptyset$
%     \item reports a random edge from $E(A, V\setminus A)$ when $E(A, V \setminus A) \neq \emptyset$.
% \end{itemize}
% Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
% \end{lemma}
% \begin{proof}
% Let us consider the sketch $S_v$ for $\mathbf{X}_v$ as guaranteed by the algorithm \Cref{lem:sketch1}. Clearly, the space complexity of the algorithm is $\Oh(n \log ^3 n)$. For $A \subseteq V(G)$, let us consider the sketch $S_A= \sum_{v \in A}S_v$. Recall that $S_v$ is the sketch for $\mathbf{X_v}$, $\mathbf{X}_A=\sum_{v \in A}\mathbf{X}_v$, and sketches are linear. So, $S_A$ is a sketch for $\mathbf{X}_A$ such that the desired properties hold (as mentioned in the statement) w.h.p.
% % The correctness for a single update follows from the $\ell_0$ sampling result\anish{which result?} by maintaining a sketch of the vector $\mathbf{X}_{{AB}}$. Hence, the lemma follows by applying the union bound over all the updates.
% \end{proof}

% %\gopi{We think that the above lemma is correct.}
% %When we insert an edge $e$ in $E(A, B)$, then $X_{{AB}}$ is changed. So, for simplicity, we say that we insert (delete) an edge $e$ to (from) the sketch of $\mathbf{X}_{{AB}}$ to mean that the sketch of $X_{{AB}}$ is updated to take care of the event that $e$ is inserted (deleted).

% \begin{lemma}\label{lem:sketch-A-B}
% %Let $A$ and $B$ be two pairwise disjoint subsets of $V(G)$. Also, let $U$ be a set of $\poly(n)$ updates to $\mathbf{X}_{{AB}}$ that is fixed by an oblivious adversary and to be revealed in a streaming fashion.
% Let $A$ and $B$ be disjoint subsets of $V(G)$.
% There exists a one-pass streaming algorithm that  stores an $\Oh(\log^3 n)$ size  sketch for $E(A,B)$ such that w.h.p. the algorithm does the following:
% \begin{itemize}
%     \item reports $\perp$ when $E(A, B)=\emptyset$
%     \item reports a random edge from $E(A, B)$ when $E(A, B) \neq \emptyset$.
% \end{itemize}
% Note that the space complexity of the algorithm is $\Oh(n \log^3 n)$.
% \end{lemma}
% \begin{proof}
%     Follows from \Cref{lem:ell0}.
% \end{proof} 

==> single-conn-proof.tex <==
\section{Missing proofs from Section \ref{sec:connect-single}}\label{app:proof-of-single-conn}

%\subsection{Proof of Lemma~\ref{lem:analysis-single}}

\begin{proof}[Proof of Lemma~\ref{lem:analysis-single}]
The query step is trivial as our algorithm stores a spanning forest and the E-tour trees. We analyze the cases for insertions and deletions separately.
%\begin{description}

      \vspace{1mm}
   \noindent    {\bf Insertion of an edge $\{u,v\}$:} As we are storing the sketches for each vertex and since the sketches are linear, the sketches of the vertices $u$ and $v$, i.e., $S_u$ and $S_v$ can be updated in $\Oh(1)$ rounds by just broadcasting the information that the sketches of $S_u$ and $S_v$ needs to be updated with insertion of edge $\{u,v\}$.
    If $C[u]=C[v]$, our algorithm does not do anything apart from updating sketches.  Now consider the case $C[u]\neq C[v]$. In this case,  we want to merge the two components $C_u$ and $C_v$. %The component id of vertices in $C_u$ and $C_v$ can be updated by broadcasting $O(1)$ information.

      \vspace{1mm}
  \noindent  {\bf Deletion of an edge $\{u,v\}$:} Note that $S_u$ and $S_v$ can be updated in $\Oh(1)$ rounds by just broadcasting the information that the sketches of $S_u$ and $S_v$ needs to be updated with deletion of edge $\{u,v\}$. If $\{u,v\}$ is not in $F$, our algorithm does not do anything apart from updating sketches. Now consider the case when $\{u,v\}$ is in $F$. We perform the Split operation for E-tours $\eu_{T}$ with both vertices $u$ and $v$ with the deletion of edge $\{u,v\}$. Let $T_u$ and $T_v$ be the two E-tours trees we obtain after the Split operation. We merge the sketches of the vertices in E-tour $\eu_{T_u}$ to get $S_{Z_u}$. This can be done by first broadcasting the id of the E-tour $\eu_{T_u}$ and then merging the sketches of the vertices in $Z_u$. Note that the broadcasting can be done in $\Oh(1)$ rounds and the merging step can be done in $\Oh(1/\spacexp)$ rounds\footnote{This is because each machine can store $\Omega(n^\spacexp / \log^3 n)$ sketches and hence we can generate the sketch $S_{Z_u}$ in $\Oh(\log_{n^\spacexp/\log ^3 n} n)=\Oh(1/\spacexp)$ rounds.}. Also, notice that the size of $S_{Z_u}$ is $\Oh(\log ^3 n)$ and can be stored in one machine. If we don't find any edge from the sketch $S_{Z_u}$, we are done. If we find an edge $\{a,b\}$ from the sketch $S_{Z_u}$, observe that it must be between $Z_u$ and $Z_v$ or equivalently one of $\{a,b\}$ is in $T_u$ and the other one is in $T_v$. Then we perform the Rooting operation to change the roots of $T_u$ and $T_v$ to $u$ and $v$, respectively. Then we execute Join operation to merge the E-tours $\eu_{T_u}$ and $\eu_{T_v}$ with insertion of edge $\{a,b\}$.  From \Cref{lem:etour-oper}, all steps required to delete edge $\{u,v\}$ can be done in $\Oh(1)$ rounds.
%\end{description}

From the above descriptions along with the fact that all the operations Rooting, Join, and Split
%, and Identify-Path
can be performed in $\Oh(1)$ rounds (\Cref{lem:etour-oper}), we conclude that each update can be performed in $\Oh(1)$ rounds.
\end{proof} 
